DeFTAN-II: Efficient Multichannel Speech Enhancement with Subgroup Processing

In this work, we present DeFTAN-II, an efficient multichannel speech enhancement model based on transformer architecture and subgroup processing. Despite the success of transformers in speech enhancement, they face challenges in capturing local relations, reducing the high computational complexity, and lowering memory usage. To address these limitations, we introduce subgroup processing in our model, combining subgroups of locally emphasized features with other subgroups containing original features. The subgroup processing is implemented in several blocks of the proposed network. In the proposed split dense blocks extracting spatial features, a pair of subgroups is sequentially concatenated and processed by convolution layers to effectively reduce the computational complexity and memory usage. For the F- and T-transformers extracting temporal and spectral relations, we introduce cross-attention between subgroups to identify relationships between locally emphasized and non-emphasized features. The dual-path feedforward network then aggregates attended features in terms of the gating of local features processed by dilated convolutions. Through extensive comparisons with state-of-the-art multichannel speech enhancement models, we demonstrate that DeFTAN-II with subgroup processing outperforms existing methods at significantly lower computational complexity. Moreover, we evaluate the model's generalization capability on real-world data without fine-tuning, which further demonstrates its effectiveness in practical scenarios.

==> Attention_analysis.tex <==
\subsection{Attention map analysis}
Fig.\,\ref{fig:att_map} illustrates the attention maps of the T-transformer using (a) CEA (Model\,4) and (b) CSA (Model\,3). These attention maps were obtained from the second head of the sixth DeFTAN-II block and depict the temporal attention within a single utterance. The attention maps were averaged across all frequency bins. The spectrograms of the clean and noisy speech, respectively, are attached below the attention maps. Several significant distinctions are discernible from the comparison of attention maps. 
%The first and third red boxes indicate that the clean spectrogram shows that the speech segments are separated based on phoneme-level distinctions. 
In contrast, the noisy spectrogram merely indicates the presence of speech due to reverberation, lacking phoneme differentiation. The attention map using CEA aptly captures the phoneme-level segregations present in the clean spectrogram, illustrated by distinctive lines. Conversely, the attention map employing CSA fails to achieve this differentiation. Furthermore, the second red box shows the presence of a non-speech click consonant. In the attention map using CEA, these non-speech click consonants can be identified through the green region positioned between the yellow-green non-speech regions, a distinction not achievable within the attention map using CSA. Thus, leveraging subgroup processing and cross-attention between features with and without local emphasis leads to a more precise mapping.
